WhisperFuzz: White-Box Fuzzing for Detecting and Locating Timing Vulnerabilities in Processors

Timing vulnerabilities in processors have emerged as a potent threat. As processors are the foundation of any computing system, identifying these flaws is imperative. Recently fuzzing techniques, traditionally used for detecting software vulnerabilities, have shown promising results for uncovering vulnerabilities in large-scale hardware designs, such as processors. Researchers have adapted black-box or grey-box fuzzing to detect timing vulnerabilities in processors. However, they cannot identify the locations or root causes of these timing vulnerabilities, nor do they provide coverage feedback to enable the designer's confidence in the processor's security. To address the deficiencies of the existing fuzzers, we present WhisperFuzz--the first white-box fuzzer with static analysis--aiming to detect and locate timing vulnerabilities in processors and evaluate the coverage of microarchitectural timing behaviors. WhisperFuzz uses the fundamental nature of processors' timing behaviors, microarchitectural state transitions, to localize timing vulnerabilities. WhisperFuzz automatically extracts microarchitectural state transitions from a processor design at the register-transfer level (RTL) and instruments the design to monitor the state transitions as coverage. Moreover, WhisperFuzz measures the time a design-under-test (DUT) takes to process tests, identifying any minor, abnormal variations that may hint at a timing vulnerability. WhisperFuzz detects 12 new timing vulnerabilities across advanced open-sourced RISC-V processors: BOOM, Rocket Core, and CVA6. Eight of these violate the zero latency requirements of the Zkt extension and are considered serious security vulnerabilities. Moreover, WhisperFuzz also pinpoints the locations of the new and the existing vulnerabilities.

==> Codes/inputs.tex <==
//Input 1
    OwnReq <= 1'b1;
    #5; //Wait for 5 cycles

//Input 2
    OwnReq <= 1'b1;
    #10; //Wait for 10 cycles
    DataResp <= 1'b1;

//Input 3
    OwnReq <= 1'b1;
    #5; //Wait for 5 cycles
    DataResp <= 1'b1;

//Input 4
    OwnReq <= 1'b1;
    #10; //Wait for 10 cycles
    DataResp <= 1'b1;

==> Codes/old_casestudy.tex <==
input own_req,data_resp,other_req,own_evict,dirty;
output [1:0] state; wire writeback;
parameter I = 2'b00,IVD = 2'b01,V = 2'b10;
assign writeback = (state == V) ? dirty:0;
    case(state)
        I: if (own_req == 1)
            state <= IVD;
        IVD: if (data_resp == 1)
            state <= V;
        V: if (other_req || own_evict) begin
                if (writeback)
                    state <= V;
                else
                    state <= I;
           end
        default: state <= I;
    endcase
...

==> Codes/tv_location/sc_boom.tex <==
1809734    if (!(state == 3'h0)) begin // @[dcache.scala 80:30]
      if (state == 3'h1) begin // @[dcache.scala 88:41]
        if (r2_data_req_fired) begin // @[dcache.scala 108:30]
          if (3'h0 == r2_data_req_cnt[2:0]) begin // @[dcache.scala 109:34]
            wb_buffer_0 <= io_data_resp; // @[dcache.scala 109:34]

==> Tables/TimVulStraDiff.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{The differences among various strategies of timing vulnerability detection.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Paper & \begin{tabular}[c]{@{}c@{}}Design\\ source\end{tabular} & \begin{tabular}[c]{@{}c@{}}Target \\ design\end{tabular} & \begin{tabular}[c]{@{}c@{}}Input \\ generation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Class \\ of vulnerability\end{tabular} & \begin{tabular}[c]{@{}c@{}}Features \\ of vulnerability\end{tabular} & \begin{tabular}[c]{@{}c@{}}Require seeds \\ with vulnerabilities?\end{tabular} & \begin{tabular}[c]{@{}c@{}}Location \\ of vulnerability?\end{tabular} \\ \hline
\osiris{}~\cite{weber2021osiris} & Black-box & Entire processor & Brute-force & eviction-based & \begin{tabular}[c]{@{}c@{}}Single-instruction, imprecise time,\\ non-specific operands\end{tabular} & No & No \\ \hline
\plumber{}~\cite{ibrahim2022microarchitectural} & Black-box & Cache module & Fuzz with manual efforts & eviction-based & Known timing vulnerabilities & Yes & No \\ \hline
\ourtool{} & RTL & Entire processor & Formalfuzz & eviction-based & General & No & Yes \\ \hline
\end{tabular}%
}
\label{tab:StraDiff}
\end{table*}

==> Tables/condition_table.tex <==
\begin{table}[]
    \centering
    \caption{Conditions of \graph{}'s edges. \ch{needs update}}
    \label{tab:conditions_casestudy}
    \begin{tabular}{c|c}
        Condition & Label \\
        tag\_address == tag[0] & C11 \\
        tag\_address == tag[1] & C12 \\
        hit == 0 \&\& full != 1 & C21 \\
        valid[0] == 1 & C22 \\
        valid[1] == 1 & C23 \\
        hit == 0 \&\& full == 1 & C31 \\
        (min\_pc > lru[way\_index] \&\& index < 1) & C32 \\
        index == cache\_ways & C33 \\
        fetch == 1 & C4\\
        complete == 1 & C5\\
    \end{tabular}
\end{table}
